TOUR: A Trajectory-Level Unlearning Benchmark for Offline Reinforcement Learning

Offline Reinforcement Learning (RL) agents are trained on fixed behavioral trajectories, which makes trajectory-level deletion important when selected data must be removed after training. Evaluating such deletion is difficult because a lower membership score can reflect trajectory removal, residual memorization visible to another attack, or policy collapse that destroys useful behavior. We introduce Trajectory-level memOrization and Unlearning in offline RL (TOUR), a benchmark that combines trajectory-level partitioning, matched non-member controls, retraining references, retained-performance anchors, and multi-attack privacy auditing. Across D4RL locomotion experiments and an exploratory AntMaze extension, TOUR shows that common deletion baselines have environment-dependent privacy-utility behavior. Retraining and fine-tuning often provide stronger retained-utility references than uniform GA+Refit, while TrajDeleter remains a useful comparator but is not uniformly stronger under the same audit. Reference-model, threshold, deviation, equivalence, action-error, representation-based, and query-limited attacks further show that a single likelihood-based membership score can overstate deletion quality. In the evaluated settings, conclusions about offline RL unlearning are therefore not stable under single-score auditing. They depend on matched non-member construction, retraining-relative calibration, attack family, retained utility, and explicit scope for diagnostic architecture or component-level evidence.

==> math_commands.tex <==
% math_commands.tex - 论文专用数学符号定义
\RequirePackage{amsmath,amssymb}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\N}{\mathbb{N}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% 数据集符号
\newcommand{\Df}{\mathcal{D}_f}          % forget set
\newcommand{\Dr}{\mathcal{D}_r}          % retain set
\newcommand{\Dn}{\mathcal{D}_n}          % matched negative set
\newcommand{\Dall}{\mathcal{D}}           % full dataset

% 策略符号
\newcommand{\pitheta}{\pi_\theta}         % 原始策略
\newcommand{\pithetap}{\pi_{\theta'}}     % unlearning 后策略
\newcommand{\pibase}{\pi_{\text{base}}}   % base 策略
\newcommand{\piretrain}{\pi_{\text{re}}} % 重训练策略

% TMI 评估符号
\newcommand{\AUCf}{\text{AUC}_f}         % forget set TMI AUC
\newcommand{\AUCr}{\text{AUC}_r}         % retain set TMI AUC
\newcommand{\privgap}{\Delta_{\text{priv}}} % privacy gap
\newcommand{\NLL}{\text{NLL}}            % negative log-likelihood

% 模型组件
\newcommand{\attn}{\text{attn}}
\newcommand{\layeri}[1]{\text{layer}_{#1}}

% KL 散度
\newcommand{\KL}{\text{KL}}

